Predictive Reduced Order Modeling of Chaotic Multi-scale Problems Using Adaptively Sampled Projections

An adaptive projection-based reduced-order model (ROM) formulation is presented for model-order reduction of problems featuring chaotic and convection-dominant physics. An efficient method is formulated to adapt the basis at every time-step of the on-line execution to account for the unresolved dynamics. The adaptive ROM is formulated in a Least-Squares setting using a variable transformation to promote stability and robustness. An efficient strategy is developed to incorporate non-local information in the basis adaptation, significantly enhancing the predictive capabilities of the resulting ROMs. A detailed analysis of the computational complexity is presented, and validated. The adaptive ROM formulation is shown to require negligible offline training and naturally enables both future-state and parametric predictions. The formulation is evaluated on representative reacting flow benchmark problems, demonstrating that the ROMs are capable of providing efficient and accurate predictions including those involving significant changes in dynamics due to parametric variations, and transient phenomena. A key contribution of this work is the development and demonstration of a comprehensive ROM formulation that targets predictive capability in chaotic, multi-scale, and transport-dominated problems.

==> Adaptivity-Formulation-old.tex <==
\subsection{Adaptive ROM formulation and practical considerations}
\label{subsec:adaptivity:algorithm}
With the \textit{predictor-corrector} approach illustrated using a linear FOM above, we now provide details on the formulation to construct adaptive ROMs for the generic dynamical system described in sec~\ref{sec:fom}, which incorporates the one-step basis adaptation (Eq.~\ref{eq:StateEstSampling:delta_basis}) and the non-local full-state evaluation (Eq.~\ref{eq:NonLocInfo:unsampled_full_state}). The construction of adaptive-ROM constitutes six major steps as follows~\footnote{The unknowns in each equation are indicated in {\color{blue} blue} }.
% we adopt a formulation that brings in non-local information to adapt the reduced spaces based on the full-state estimate evaluated at the current time step, $n$, $\solPrimFOMAdaptive^{\iterIdx}$. %While the frequency of on-line basis updates is variable in ~\citep{PeherstorferADEIM}, we choose to adapt the basis at each time step, inspired by the predictor-corrector approach.  
% The sampling points are adapted every $z_s$ time step, which is an empirical parameter. The algorithm (at every time step) for a general non-linear multi-scale transport problem is presented as follows~\footnote{The unknowns in each equation are indicated in {\color{blue} blue} }. 

\noindent \underline{\textbf{Step 0}: \textit{Initialize basis and sampling points}}

The FOM (Eq.~\ref{eq:fom_linear_multi_discrete}) is solved for a small number of time steps, $w_\text{init} \in \mathbb{N}$ to obtain a collection of full states, $\mathbf{Q}_p^\text{init} = \left[ \solPrimFOM^1 , \ldots , \solPrimFOM^{w_\text{init}} \right]$, which is then used to determine the initial basis, ${\color{blue}\trialBasisPrim^0}$, via POD as described in sec~\ref{subsec:pod} and sampling points, ${\color{blue}\sampMat_{0}}$, using gappy POD~\citep{gappyPOD}. It needs to be remarked that though this step can be considered as an \textit{offline} stage, $w_\text{init}$ is typically negligible compared to the total number of time steps, $K \in \mathbb{N}$, for the \textit{online} stage calculations (i.e. $w_\text{init} \ll K$), therefore significantly reducing the \textit{offline} computational cost that involves solving the expensive FOM to collect the full-state information for the \textit{offline/online} ROM methods~\citep{HuangMPLSVT2022,Barnett_QuadraticPROM2022,McQuarrieOpInf2021}. Moreover, the number of time steps for initial FOM simulation, $w_\text{init}$, is one hyper-parameter in the formulation, the effects of which are investigated further in sec~\ref{subsec:1d:sensitivity_arom}. 

Furthermore, once the initial basis and sampling points are established in this initialization step, no additional \textit{offline}-stage FOM simulation is necessary to construct ROMs for another parameter. This arguably ``no \textit{offline} stage" feature inherently enables parametric predictive capabilities in the resulting adaptive ROMs~\citep{PeherstorferADEIM,Ramezanian_2021_OnTheFlyROM}, thus avoiding the common challenges in developing \textit{parametric} ROMs~\citep{Benner_Gugercin_Willcox_PMR2015}, especially for chaotic convenction-dominanted problems exhibiting the Kolmogorov barrier.

After this initialization step, the following steps are operated in the \textit{online} stage.

\noindent \underline{\textbf{Step 1}: \textit{Propagate reduced states}}

Following the formulation in sec~\ref{subsec:hyper_reduction}, hyper-reduced MP-LSVT ROM is constructed and solved to propagate the reduced states in time from $\solPrimROMRed^{\iterIdx-1}$ to $\solPrimROMRed^{\iterIdx}$
\begin{equation}
    \lp \sampMat^T_{n-1} \testBasisPrim^\iterIdx \rp^T \left[ \lp \sampMat^T_{n-1} \resBasis \rp^{+} \right]^T \lp \sampMat^T_{n-1} \resBasis \rp^{+} \sampMat^T_{n-1} \scaleMatCons \resFunc{ {\color{blue}\Tilde{\mathbf{q}}^n} } = \zeroVec,
\end{equation}
where $ {\color{blue}\Tilde{\mathbf{q}}^n} = \solPrimFOMRef + \scaleMatPrim^{-1} \trialBasisPrimN{\iterIdx-1} {\color{blue}\solPrimROMRed^{\iterIdx}}$. For the ease of practical considerations, $\resBasis = trialBasisPrimN{\iterIdx-1}$, since it is found to provide excellent approximations in the hyper-reduction~\citep{HuangMPLSVT2022}.

\noindent \underline{\textbf{Step 2}: \textit{Estimate full states at \textbf{sampled} points}}

Evaluate the state estimate at sampled points
\begin{equation}
    \begin{aligned}
        \sampMat^T_{n-1}\solConsFOMFunc{\sampMat_{n-1}{\color{blue}\sampMat^T_{n-1}\solPrimFOMAdaptive^\iterIdx}+\sampMat_{n-1}^{\ast}\sampMat^{\ast T}_{n-1}\solPrimROMFull^{\iterIdx}, \timeVar^\iterIdx} & + \sum^{\itermaxLinMS}_{j=1} \alpha_j \sampMat^T_{n-1}\solConsFOMFunc{\solPrimROMFull^{\iterIdx-j}} \\
        - \dt \beta_0 \sampMat^T_{n-1}\rhsFunc{\sampMat_{n-1}{\color{blue}\sampMat^T_{n-1}\solPrimFOMAdaptive^\iterIdx}+\sampMat_{n-1}^{\ast}\sampMat^{\ast T}_{n-1}\solPrimROMFull^{\iterIdx}, \timeVar^\iterIdx} &- \dt \sum^{\itermaxLinMS}_{j=1} \beta_j \sampMat^T_{n-1}\rhsFunc{\solPrimROMFull^{\iterIdx-j}, \timeVar^{\iterIdx-j}} = 0. 
    \end{aligned}
\end{equation}
% Collect full-state information at the sampled points:
% \begin{equation}
%     \mathbf{F}_S = \left[ \sampMat^T_{n-1}\solPrimFOMAdaptive^{\iterIdx-w-1} \ldots \sampMat^T_{n-1}\solPrimFOMAdaptive^{\iterIdx} \right] \in \mathbb{R}^{
%     \numSamps \times w}.
% \end{equation}

\noindent \underline{\textbf{Step 3}: \textit{Estimate full states at \textbf{unsampled} points}} 

 Update state estimate at unsampled points every $z_s$ time steps.
\begin{equation}
    \begin{aligned}
        \sampMat^{\ast T}_{n-1}  \solConsFOMFunc{\sampMat_{n-1}\sampMat^T_{n-1}\solPrimFOMAdaptive^\iterIdx+\sampMat_{n-1}^{\ast}{\color{blue}\sampMat^{\ast T}_{n-1}\solPrimFOMAdaptive^\iterIdx}, \timeVar^\iterIdx} &+ \sum^{\itermaxLinMS}_{j=1} \alpha_j  \sampMat^{\ast T}_{n-1} \solConsFOMFunc{\solPrimROMFull^{\iterIdx-j \cdot z_s}} \\ 
        - z_s \dt \beta_0  \sampMat^{\ast T}_{n-1}\rhsFunc{\sampMat_{n-1}\sampMat^T_{n-1}\solPrimFOMAdaptive^\iterIdx+\sampMat_{n-1}^{\ast}{\color{blue}\sampMat^{\ast T}_{n-1}\solPrimFOMAdaptive^\iterIdx}, \timeVar^\iterIdx} &- z_s \dt \sum^{\itermaxLinMS}_{j=1} \beta_j  \sampMat^{\ast T}_{n-1} \rhsFunc{\solPrimROMFull^{\iterIdx-j\cdot z_s}, \timeVar^{\iterIdx-j\cdot z_s}} = 0. 
    \end{aligned}
\end{equation}

% Collect the full-state estimate at all the grid points: 
% \begin{equation}
%     \mathbf{F} = \left[ \solPrimFOMAdaptive^{\iterIdx-w-1} \ldots \solPrimFOMAdaptive^{\iterIdx} \right] \in \mathbb{R}^{\numDOF \times w}.
% \end{equation}

\noindent \underline{\textbf{Step 4}: \textit{Update the basis} ($\trialBasisPrimN{n}$)}

If \emph{not} updating  sampling points, the basis is updated only at the sampled points
\begin{equation}
   {\color{blue} \sampMat^T_{n-1}\trialBasisPrimN{n}} = \sampMat^T_{n-1}\trialBasisPrimN{n-1} + \frac{ \lp  \sampMat^T_{n-1}\solPrimFOMAdaptive^n - \sampMat^T_{n-1}\solPrimROMFull^n \rp (\solPrimROMRed^n)^T}{||\solPrimROMRed^n||_2^2} ,
\end{equation}

If updating the sampling points (i.e. every $z_s$ time-steps), the basis is updated at all grid points
\begin{equation}
  {\color{blue}  \trialBasisPrimN{n}} = \trialBasisPrimN{n-1} + \frac{ \lp \sampMat_{n-1} \sampMat^T_{n-1}\solPrimFOMAdaptive^n + \sampMat_{n-1}^\ast \sampMat^{\ast T}_{n-1}\solPrimFOMAdaptive^n - \solPrimROMFull^n \rp (\solPrimROMRed^n)^T}{||\solPrimROMRed^n||_2^2},
\end{equation}

\noindent \underline{\textbf{Step 5}: \textit{Update the sampling points} ($\sampMat_{n}$)}

Update sampling points every $z_s$ time steps ($\sampMat_{n-1}$ to $\sampMat_n$) such that the interpolation error below is minimized

\begin{equation}
   {\color{blue} \sampMat_{n}} =  \argmin_{\sampMat^*} \norm{ \solPrimFOMAdaptive^n - \trialBasisPrim^n \lp \sampMat^{*T} \trialBasisPrim^n \rp^{+} \sampMat^{*T} \solPrimFOMAdaptive^n }^2,
   %{\color{blue} \sampMat_{n}} =  \argmin_{\sampMat^*} \norm{ \mathbf{F} - \trialBasisPrim^n \lp \sampMat^{*T} \trialBasisPrim^n \rp^{+} \sampMat^{*T} \mathbf{F} }^2,
\end{equation}
where for practical and scalable and implementations, the norm $\norm{ \solPrimFOMAdaptive^n - \trialBasisPrim^n \lp \sampMat^{*T}_{n-1} \trialBasisPrim^n \rp^{+} \sampMat^{*T}_{n-1} \solPrimFOMAdaptive^n }^2$ is evaluated  and $\sampMat_n$ is selected based on the locations that correspond to the largest contributions to the norm.

\subsubsection{Computational procedures and complexity of adaptive ROM}
Next, we provide a detailed computational complexity analysis of the adaptive ROM algorithm in terms of floating-point operations (FLOPs). Here, a FLOP refers to any floating-point addition or
multiplication; no distinction is made between the computational cost of either operation.



\begin{table}
\centering
\begin{tabular}{ll} 
\toprule
\textbf{Operations} & \textbf{Approximate FLOPs} \\
\midrule
\textbf{Step 1}: Propagate reduced variables & $[(z_s p_1)/{\lambda}] \text{FLOPs}_\text{FOM}$ \\
\textbf{Step 2}: State estimate at sampled points & $p_2 \text{FLOPs}_\text{FOM}$ \\
\textbf{Step 3}: State estimate at unsampled points & $[( z_s - 1 ) p_2 ( n_s / N_c )] \text{FLOPs}_\text{FOM}$ \\
\textbf{Step 4}: Basis update & $[n_v N_c + (z_s - 1)n_v n_s + z_s](4m-1)$ \\
\textbf{Step 5}: Sampling points update & $\nu n_v N_c$ \\
\midrule
Total & $ [(z_s p_1)/{\lambda} + p_2 + ( z_s - 1 ) p_2 ( n_s / N_c )] \text{FLOPs}_\text{FOM} $ \\
& $+ [n_v N_c + (z_s - 1)n_v n_s + z_s](4m-1) + \nu n_v N_c$ \\
\bottomrule
\end{tabular}
\caption{\label{table:flops_adaptiveROM} Approximating floating-point operations for $z_s$ time steps and $K$ subiterations (in total) within each time step for adaptive ROM with $p_2$ subiterations used for state estimate while $p_1$ used for ROM.}
\end{table}

\begin{equation}
    \lambda_\text{AROM} = \frac{\text{FLOPs}_\text{FOM}}{\text{FLOPs}_\text{AROM}} < z_s \frac{K}{p_2}
    % \lambda_\text{AROM} & = \frac{\text{FLOPs}_\text{FOM}}{\text{FLOPs}_\text{AROM}} \\ & = \frac{z_s K}{[(z_s p_1)/{\lambda} + p_2 + ( z_s - 1 ) p_2 ( n_s / N_c )] + O\left( [n_v N_c + (z_s - 1)n_v n_s + z_s]K(4m-1) \right) + \nu n_v K N_c} \\ & < z_s \frac{K}{p_2}
    \label{eq:adaptiveROM_efficiency_gain}
\end{equation}

\begin{figure}
	\centering
	\includegraphics[width=0.6\textwidth]{./figures/FLOPs_AdaptiveROM_vs_zs.png}
	\caption{Approximate efficiency gain of adaptive ROM versus sampling points.}
    \label{fig:flops_arom} 
\end{figure}




==> Proofs.tex <==
\section{Stability
of Least-Squares-based ROMs for Linear Problems}
\label{proof}
In this section, we provide a complete proof of least-squares-based ROMs for a linear time-invariant (LTI) system. While the finite element community is rich with literature on the analysis of least-squares-based techniques (e.g.~\cite{LSFEM}), stability analysis in the ROM literature is not commonly found. Pursuing a viewpoint of contractivity, stability preservation for projection-based model order reduction in continuous time is presented in ~\cite{Selga_stabilityPreservation2012}. In contrast, we pursue a linear algebra standpoint in discrete time, which will be useful for the analysis of numerical results in Section~\ref{2d:LinearStability}.

For the full order model, we assume an autonomous LTI system given by
\begin{equation}
    \frac{\text{d} \solConsFOM}{\dTimeVar} = \ltiMatA \solConsFOM, \ \ \solConsFOM(0) = \solConsFOM_0,
    \label{LTI}
\end{equation}
where $\solConsFOM \in {\mathbb{R}^{\numDOF}}$, and $\ltiMatA \in \mathbb{R}^{\numDOF \times \numDOF}$. 
For clarity of presentation, we will consider a backward Euler discretization for the FOM:

\begin{align}
  \solConsFOM^\iterIdx  &= (\mb{I} - \dt \ltiMatA)^{-1} \solConsFOM^{\iterIdx-1}, \ \  \solConsFOM^0 = \solConsFOM_0.
  \label{LTI:discrete}
\end{align}

Consider a low-rank representation $\solConsROMFull(\timeVar) \triangleq \trialBasisCons \solConsROMRed(\timeVar)$, where $\trialBasisCons \in \mathbb{R}^{\numDOF \times \numSolModes}$ and $\solConsROMRed \in \mathbb{R}^{\numSolModes}$. Note that the main conclusions also hold when $\solConsROMFull (\timeVar) \triangleq \solConsFOMRef + \scaleMatCons^{-1} \trialBasisCons \solConsROMRed (\timeVar)$.

\subsection{Least-Squares Petrov Galerkin ROM}
Following the development in Section~\ref{slspg_rom}, we get
\begin{equation}
\testBasisCons^T \frac{ \solConsROMFull^\iterIdx - \solConsROMFull^{\iterIdx-1} }{\dt} =  \testBasisCons^T \ltiMatA \solConsROMFull^\iterIdx,
\label{LTI:ROMT}
\end{equation}
where $\testBasisCons \triangleq (\mb{I} - \dt \ltiMatA) \trialBasisCons.$ Manipulating further, we get the governing equations for the modal coefficients in the form
\begin{equation}
(\testBasisCons^T \testBasisCons) \solConsROMRed^\iterIdx =  \testBasisCons^T \trialBasisCons \solConsROMRed^{\iterIdx-1}, \ \ \solConsROMRed^0 = \trialBasisCons^T \solConsFOM_0.
\label{LTI:ROM}
\end{equation}
 We will now prove the stability of the ROM (Eq.~\ref{LTI:ROM}) under the condition that the FOM (Eq.~\ref{LTI:discrete}) is linearly stable. 

We will pursue a notion of stability via the Euclidean vector-induced matrix norm $\norm{\cdot}.$ We will use $\sigma_\genIdx(\mb{A})$ to represent the $\genIdx^{th}$ singular value of a matrix $\mb{A}$. For a real symmetric matrix $\mb{S}$, we will use $\lambda_\genIdx(\mb{S})$ to represent the $\genIdx^{th}$ eigenvalue of $\mb{S}$, with the  eigenvalues arranged in descending order.

\vspace{0.75cm}

\noindent{\bf Theorem 1} : If the FOM given by Equation~\ref{LTI:discrete} is asymptotically stable in the sense of $\norm{(\mb{I} - \dt \ltiMatA)^{-1}} \leq 1$, then the ROM given by Equation~\ref{LTI:ROM} is also asymptotically stable with no further assumptions required.
\vspace{0.25cm}
\noindent {\em Proof}:
The problem statement reduces to showing that
\begin{equation}
\norm{(\testBasisCons^T \testBasisCons)^{-1} \testBasisCons^T \trialBasisCons}  \leq 1,
\end{equation}
with $\testBasisCons\triangleq \ltiMatB\trialBasisCons$, where $\ltiMatB \triangleq \mb{I} - \dt \ltiMatA$, given $\norm{\ltiMatB^{-1}} \leq 1.$

Since $\ltiMatB$ and $\trialBasisCons$ are both full-rank matrices, $\testBasisCons$ is also a full-rank matrix, and the left pseudo-inverse $\testBasisCons^+ \triangleq (\testBasisCons^T \testBasisCons)^{-1} \testBasisCons^T$ also exists. Therefore, given $\norm{\testBasisCons^+}= \frac{1}{\sigma_{\numSolModes}(\testBasisCons)}$ we have 
\begin{equation}
 \norm{(\testBasisCons^T \testBasisCons)^{-1} \testBasisCons^T \trialBasisCons} = \norm{\testBasisCons^+   \trialBasisCons} \leq  \norm{\testBasisCons^+} \norm{\trialBasisCons}
 = \frac{1}{\sigma_{\numSolModes}(\testBasisCons)}
 \label{eq:proof}
\end{equation}
and thus our problem reduces to showing 

\begin{equation}
    \sigma_{\numSolModes}(\testBasisCons) = \sigma_{\numSolModes}(\ltiMatB \trialBasisCons) \geq 1, \ \ \textrm{given} \ \ \sigma_{\numDOF}(\ltiMatB) \geq 1.
    \label{eq:neweq}
\end{equation}


We write $\testBasisCons^T \testBasisCons = \trialBasisCons^T \ltiMatB^T \ltiMatB \trialBasisCons$
and use the Poincar\'{e} separation theorem~(\ref{appendix:poincare})  which yields
\begin{equation}
\lambda_{\numSolModes}(\testBasisCons^T \testBasisCons) \geq \lambda_{\numDOF} (\ltiMatB^T \ltiMatB).
\end{equation}
Since $\lambda_{\numSolModes}(\testBasisCons^T \testBasisCons) = \sigma_{\numSolModes}(\testBasisCons)$ and  $\lambda_{\numDOF}(\ltiMatB^T \ltiMatB) = \sigma_{\numDOF}(\ltiMatB)$, we have
\begin{equation}
\sigma_{\numSolModes}(\testBasisCons) \geq \sigma_{\numDOF} (\ltiMatB).
\end{equation}
Since $\sigma_{\numDOF} (\ltiMatB) \geq 1$, we have $\sigma_{\numSolModes}(\testBasisCons) \geq 1$. This completes the proof following Equation~\ref{eq:proof}. 

\vspace{0.75cm}

\subsection{Galerkin ROMs}

Galerkin projection  on Eq.~\ref{LTI:discrete} yields
\begin{equation}
(\mb{I} - \dt \trialBasisCons^T \ltiMatA \trialBasisCons)\solConsROMRed^\iterIdx = \solConsROMRed^{\iterIdx-1}.
\label{LTI:ROMG}
\end{equation}
Stability demands $\norm{(\mb{I} - \dt \trialBasisCons^T \ltiMatA \trialBasisCons)^{-1}} \leq 1$. This can be written as $\norm{(\trialBasisCons^T \ltiMatB \trialBasisCons)^{-1}} \leq 1$, with $\ltiMatB \triangleq \mb{I} - \dt \ltiMatA$. 

$\bullet$ If $\ltiMatA$ is a symmetric matrix, $\norm{(\trialBasisCons^T \ltiMatB \trialBasisCons)^{-1}} = \frac{1}{\lambda_{\numSolModes}(\trialBasisCons^T \ltiMatB \trialBasisCons)}$. Also note that $\ltiMatA$ is negative definite, $\ltiMatB$ will be positive definite. Thus, we have
\begin{equation}
\lambda_{\numSolModes}(\trialBasisCons^T \ltiMatB \trialBasisCons) \geq \lambda_{\numDOF}(\ltiMatB) \geq 1,
\end{equation}
where the first inequality is due to the Poincar\'{e} separation theorem, and the second one is due to the fact that $\ltiMatA$ is negative-definite. Thus, given that the FOM is asymptotically stable, the Galerkin ROM is asymptotically stable with no further assumptions required.

$\bullet$ If $\ltiMatA$ is not a symmetric matrix, then $\norm{(\trialBasisCons^T \ltiMatB \trialBasisCons)^{-1}} = \frac{1}{\sigma_{\numSolModes}(\trialBasisCons^T \ltiMatB \trialBasisCons)}$ and thus we have to show that $\sigma_{\numSolModes}(\trialBasisCons^T \ltiMatB \trialBasisCons) \ge 1$. While a convenient upper bound exists (refer~\ref{appendix:singValIdent}) $\sigma_{\numSolModes}(\trialBasisCons^T \ltiMatB \trialBasisCons) \leq \sigma_{\numSolModes}(\ltiMatB)$,  tight lower bounds do not exist for general non-symmetric $\ltiMatB$. Thus unconditional stability (or instability) cannot be proven, and a case-by-case approach is required, depending on the structure of $\ltiMatA$ and the time-step $\dt$.  It should, however, be noted that, even when the FOM represents a discretization of Hyperbolic PDEs, the underlying numerical dissipation in the FOM, coupled with a small time-step $\dt$ can stabilize Galerkin ROMs depending on the level of mode truncation.


\vspace{0.75cm}

\noindent{\bf Theorem 2} : If the FOM given by Equation~\ref{LTI:discrete} is asymptotically stable in the sense of $\norm{(\mb{I} - \dt \ltiMatA)^{-1}} \leq 1$, then the Galerkin ROM given by Equation~\ref{LTI:ROMG} is also asymptotically stable if $\lambda_{\numDOF}\left( \mb{I} - \frac{1}{2} \dt (\ltiMatA + \ltiMatA^T)\right) \geq 1.$



\vspace{0.25cm}
\noindent {\em Proof:} Define $\ltiMatB \triangleq \mb{I} - \dt \ltiMatA$. The goal is to show $\sigma_{\numSolModes}(\trialBasisCons^T \ltiMatB \trialBasisCons) \geq 1.$

From~\ref{appendix:evalsHermitian}, 
\begin{equation}
\sigma_\genIdx(\trialBasisCons^T \ltiMatB \trialBasisCons) \geq \lambda_\genIdx \left(\trialBasisCons^T \frac{\ltiMatB + \ltiMatB^T}{2} \trialBasisCons \right)
\end{equation}

From~\ref{appendix:poincare}, 
\begin{equation}
\lambda_\genIdx \left(\trialBasisCons^T \frac{\ltiMatB + \ltiMatB^T}{2} \trialBasisCons  \right) \geq \lambda_{\numDOF - \numSolModes +\genIdx} \left(\frac{\ltiMatB + \ltiMatB^T}{2}\right).
\end{equation}

Therefore
\begin{equation}
\sigma_{\numSolModes}(\trialBasisCons^T \ltiMatB \trialBasisCons) \geq \lambda_{\numDOF} \left( \frac{\ltiMatB + \ltiMatB^T}{2}\right)
\end{equation}
and stability demands
\begin{equation}
\lambda_{\numDOF} \left(\frac{\ltiMatB + \ltiMatB^T}{2}\right) \geq 1.
\end{equation}
\vspace{0.75cm}

\noindent Note: It can be easily verified, for instance, that a Galerkin ROM of a linear upwind spatial discretization of the linear advection equation with Euler implicit time integration is unconditionally stable. 

%\begin{comment}
%\noindent Note: The above condition is not too restrictive.
%Consider $$\frac{\partial u}{\partial t}+a \frac{\partial u}{\partial x}=0.$$
%Defining $\nu \triangleq a \frac{\Delta t}{\Delta x}$, Euler Implicit with first order upwind yields
%$$\mb{B} = \mb{T}[-\nu,1+\nu,0], $$ where $\mb{T}$ represents a tridiagonal matrix with lower diagonal $-\nu,$ diagonal $1+\nu$ and upper diagonal element $0.$ In the periodic case, $\lambda_n\left( \frac{\mb{B}+\mb{B}^T}{2}\right) = 1.$ In the non-periodic case, $\lambda_n\left( \frac{\mb{B}+\mb{B}^T}{2}\right) = 1+\nu \epsilon$, where $\epsilon > 0 $ is related to the mesh resolution. The Galerkin ROM is unconditionally stable in both cases.

%\noindent Note: Galerkin projection on the above problem yields
%\begin{equation}
%\mb{V}^T \frac{ \tilde{\mb{q}}^n - \tilde{\mb{q}}^{n-1} }{\Delta t} =  %\mb{V}^T \mb{J} \tilde{\mb{q}}^n,
%\label{LTI:ROMTG}
%\end{equation}
%which yields 
%\begin{equation}
%(\mb{I}-\Delta t \mb{V}^T \mb{J}\mb{V})\mb{q}_r^n =   \mb{q}_r^{n-1}.
%\label{LTI:ROMG}
%\end{equation}
%Stability demands $\norm{(\mb{I}-\Delta t \mb{V}^T \mb{J} \mb{V})^{-1}} \leq 1$. This can be written as $\norm{(\mb{V}^T \mb{B} \mb{V})^{-1}} \leq 1$, with $\mb{B} \triangleq \mb{I}-\Delta t \mb{J}$. 

%$\bullet$ If $\mb{J}$ is a symmetric matrix, $\norm{(\mb{V}^T \mb{B} \mb{V})^{-1}} = \frac{1}{\lambda_k(\mb{V}^T \mb{B} \mb{V})}$. Also note that $\mb{J}$ is negative definite, $\mb{B}$ will be positive definite. Thus, we have $$\lambda_k(\mb{V}^T \mb{B} \mb{V}) \geq \lambda_n(\mb{B}) \geq 1,$$ where the first inequality is due to the Poincare separation theorem, and the second one is due to the fact that $\mb{J}$ is negative-definite. Thus, given that the FOM is asymptotically stable, the Galerkin ROM is asymptotically stable with no further assumptions required.

%$\bullet$ If $\mb{J}$ is not a symmetric matrix, then $\norm{(\mb{V}^T \mb{B} \mb{V})^{-1}} = \frac{1}{\sigma_k(\mb{V}^T \mb{B} \mb{V})}$ and thus we have to show that $\sigma_k(\mb{V}^T \mb{B} \mb{V}) \ge 1$. While a convenient upper bound exists (refer~\ref{appendix:poincare}) $\sigma_k(\mb{V}^T \mb{B} \mb{V}) \leq \sigma_k(\mb{B})$,  tight lower bounds do not exist for general non-symmetric $\mb{B}$. Thus unconditional stability (or instability) cannot be proven, and a case-by-case approach is required, depending on the structure of $\mb{J}$ and the time-step $\Delta t$.  It should, however, be noted that, even when the FOM represents a discretization of Hyperbolic PDEs, the underlying numerical dissipation in the FOM, coupled with a small time-step $\Delta t$ can stabilize Galerkin ROMs depending on the level of mode truncation.


%\begin{comment}
%We prove such a result below.

%\vspace{0.75cm}
%\noindent{\bf Theorem 2} : If the time step $\Delta t$ is chosen such that $ \norm{\Delta t \mb{J}} \leq \alpha$, then the Galerkin ROM given by Equation~\ref{LTI:ROMG} is asymptotically stable in the sense of $\norm{(\mb{I} - \Delta t \mb{V}^T \mb{J} \mb{V})^{-1}} \leq 1$ with no further assumptions required.
%\vspace{0.25cm}
%\noindent {\em Proof:} Since $\norm{\Delta t \mb{J}} \le 1,$ we have $\sigma_1(\Delta t \mb{V}^T  \mb{J} \mb{V}) \leq \sigma_1(\Delta t \mb{J})$. This inequality is because of a singular value transformation identity (refer~\ref{appendix:poincare}). Since $\sigma_1(\Delta t \mb{V}^T  \mb{J} \mb{V}) < 1$, we have $\norm{} < 1$
%\vspace{0.75cm}

%\end{comment}

%\end{comment}

%\clearpage Thus, for non-symmetric $\mb{B}$, the Galerkin method may be stable or unstable on a case-by-case basis. It is not necessary that a Galerkin ROM developed from discretizations of Hyperbolic PDEs would be unstable, because the dissipation terms present in the FOM can stabilize the ROM.

==> Reviewer1.tex <==
\section*{Reviewer 1}

The authors introduce a new adaptive model reduction approach, modeled off the work of Peherstorfer (2020), that breaks the traditional offline/online decomposition of model reduction. While this sacrifices speedup potential relative to static model reduction, it can improve the predictive capability and parametric robustness of reduced-order models, particularly in convection-dominated problems whose reduction potential is limited by the slowly decaying Kolmogorov n-width. This method is novel and addresses the most fundamental limitation of projection-based model reduction and is therefore highly pertinent. The paper is well-written and provides an in-depth literature review, and clearly states how the current work relates to other approaches. The paper has a few fundamental issues that should be addressed before publication.

\addrOne{We thank the reviewer for the comments and have addressed all of them in the paper highlighted in color brown.}

\begin{enumerate}
    \item Because Section 2 mentions that the FOM can be solved with multistage methods (like Runge-Kutta), the authors should discuss how the proposed method could be used with multistage time stepping. It is not obvious how (or if) the predictor-corrector approach would work in this setting.

    \addrOne{The formulation of the MP-LSVT ROM  with multistage times stepping was  discussed in the previous paper "C. Huang, C. R. Wentland, K. Duraisamy, C. Merkle, Model reduction for multi-scale transport problems using model-form preserving least-squares projections with variable transformation, Journal of Computational Physics 448." Given the present paper is already very long, we did not include the details for the compactness of the current paper. As for the predictor-corrector approach in the adaptive ROM algorithm, the major part that involves time stepping method is Eqs.(40) and (41). We have included additional discussions in that section to cover the multistage methods.}
    

    \item Is the MV-LSVT approach still necessary with the new adaptive basis/sampling, or could a simple Galerkin approximation using the conserved state work equally well? A brief numerical experiment with the laminar flame could provide insight into this. If the answer is positive, it would make an even stronger case for the adaptive approach.
    
    \addrOne{We thank the reviewer for bringing this up. In our preliminary tests, Galerkin + adaptive ROMs were confirmed to provide more accurate results than Galerkin ROMs. However, Galerkin ROMs were almost always found to be unstable, even with adaptivity, especially with larger $z_s$.  We have not performed extensive investigations but preliminary analysis indicates that the MP-LSVT approach is necessary because it provides a reduced-state solution, $\mathbf{q}^{n-1}_r$, that satisfies Eq.(16). Also, Given the length of the current paper, we hope to include this study in a future publication.}


    \item The size of the sampling matrix $\mathbf{S}$ in 4.1.1 is not given. I assume it is $N \times n_s$ (like in the beginning of Section 4). However, if this is the case, the definition of $\mathbf{S}^{*}$ as $\mathbf{S}^{*} = \mathbf{I} - \mathbf{S}$  does not make sense because the size of the identity matrix ($N \times N$) and $\mathbf{S}$ ($N \times n_s$) are incompatible.
    
    \addrOne{Thank you for pointing this out. The size of sampling matrix $\mathbf{S}$ is given under Eq.(12) while the size of the unsampling matrix $\mathbf{S}^{*}$ is $N \times (N-n_s)$ and should be the set difference between $\mathbf{S}$ and $\mathbf{I}$. We have corrected it in 4.1.1 above Eq.(25).}


    \item At the end of 4.1.2, the authors state "Eq. 35 implies a much smaller magnitude of error compared to Eq. 29". Additional explanation is needed here because both of these equations are complicated and involve non-intuitive terms.

    \addrOne{Thank you for pointing this out. We have revised that section to reflect the reviewer's comment.}


    \item In Eqn. 38, the minimization problem uses an updated reduced basis ($V + \delta V$) with previously computed ROM coefficients. Shouldn't an updated reduced basis require the reduced coordinates to be updated? Please explain.

    \addrOne{The original problem setup is to update the reduced states, basis, and the sampling points simultaneously based on the minimization problem in Eq.(16). However, as stated in the paper, solving Eq.(16) leads to intractable problem and therefore we seek to solve the problem sequentially, which first solves the reduced states and then update the basis.}
    

    \item Additional detail should be provided on how the unknown blue terms can be computed in Eqns. (40) and (41) as it is not obvious. Furthermore, even if those systems are solved for the blue terms, the unsampled points appear to be frozen at the state reconstructed from the reduced-order model prior to the basis correction. This could be provided inaccurate "boundary" information for the sampled points and lead to substantial error. Additional discussion of this issue should be included.

    \addrOne{We have included additional discussion regarding how the blue terms are computed in Eqs.(40) and (41). The estimated full states at the unsampled points remain unchanged when evaluating the full states at the sampled points in Eq.(40) but it needs to be highlighted that they do get updated in Eq.(41) with a larger physical time step and the dynamics at the unsampled points evolve slower than those at the sampled points so the effects of "frozen" unsampled points are expected to be not significant but will be dependent on the selection of $z_s$. We have included more discussion on this as well.}
    

    \item The strategy of only updating the sampling points every $z_s$ time steps seems to be a limitation of the overall method. Provide a discussion of the classes of problems the authors expect this would and would not work well. For example, I expect problems with strong, propagating shocks would require a small $z_s$ and limit speedups.

    \addrOne{As emphasized in the paper, the selection of $z_s$ is a determinant factor for the performance of the adaptive ROM and it is formulated based on the observations that local coherence features fast dynamics while non-local coherence features slow dynamics, which is applicable to a majority class of problems. We argue that the new adaptive ROM formulation might encounter limitations in problems featuring similar fast (or slow) dynamics for local and non-local coherence. For propagating strong shocks, the adaptive ROM has been demonstrated to provide reasonable speedups already without accounting for the non-local information by Peherstorfer~\cite{PeherstorferADEIM} and we have demonstrated our new method for detonation wave problems recently (to be published soon). We have provided relevant discussions in the revision in sec 4.2.1.}
    

    \item In the numerical experiments, the authors get a "free" factor of 2 by using half as many pseudo iterations for the ROM and full-state estimation than used for the FOM. This is only justified if the authors can show the accuracy or robustness of the FOM degrades if half as many pseudo iterations were used. Otherwise, it is unfairly padding the speedups by artificially making the FOM take twice as much time.

    \addrOne{For all the test cases in the current paper, we have verified that all the FOM solutions converge to machine zero (i.e. the FOM equation residual goes to zero in Eq.~\ref{eq:fom_linear_multi_discrete}) with the designated number of pseudo iterations while using less iterations can lead to non-zero FOM equation residual, which indicates errors in the FOM solutions.}


    \item The parameter $z_s$ seems likely to scale inversely proportional to time step size (e.g., if dt reduced by a factor of 2, then $z_s$ could be increased by a factor of 2). And because $z_s$ is so fundamental to the speedup of the method, the authors should justify the choice of dt for both problems. For example, dt = 0.01 microseconds for the laminar flame (6000 time steps for a 60 microsecond simulation) seems extremely small given the authors are using a 2nd order implicit scheme. A more realistic time step could necessitate less aggressive choices for $z_s$, which could further limit the speedup. A numerical experiment that demonstrates the most appropriate dt for the FOM for each experiment would be a convincing way to settle this question.

    \addrOne{This is a good point. However, given the requirement to resolve the dynamics of the flame and the extreme stiffness of chemically reacting flows, even implicit schemes require small time steps. Our test problems selected are well-established and have been used for ROM development and investigations in several publications.We refer the reviewer to Refs.~\cite{HuangMPLSVT2022,Huang2020_SpeciesLimiters,HuangAIAAJ2019} for additional detail.}
    

    \item Please indicate in the manuscript whether the speedups are computed by directly timing the code, or using the formulas derived the complexity analysis section.
    
    \addrOne{The speedups are computed by directly timing the code and we have highlighted this at the end of page 17 in the paper.}
    
\end{enumerate}


==> Reviewer2.tex <==
\section*{Reviewer 2}

The present paper describes a method for 'online adaptation of basis and sampling' of reduced order models with the goal of making them truly predictive beyond, and even far beyond, the training window for problems of considerable physical complexity. The approach uses projection methods based upon POD bases and employs a slightly modified version of the classical LSPG method. A relatively benign one-dimensional example is used to show the difficulties static bases encounter and to justify the need for dynamic bases that adapt as the solution progresses. The primary focus of the paper is on identifying methods for achieving the needed basis adaptations in an efficient manner. The paper provides a careful and complete description of the adaptation procedure and culminates with several examples of impressive long-term predictions for problems of considerable complexity. The paper is well written and complete, details are nicely relegated to brief appendices, and overall, the work represents an important contribution to stable, predictive roms. I support its publication. My comments are relatively minor but should be incorporated before publication to clarify and strengthen the paper.

\addrTwo{We thank the reviewer for the comments and have addressed all of them in the paper highlighted in color blue. Additionally, we would like to point out that the 1D problem - while simple when considered in isolation - is highly challenging for contemporary projection-based ROMs because of the advection, and the requirement of prediction well outside the training window. In fact, static basis ROMs cannot be used for this problem.}

My first concern is with the overuse of the word 'chaotic' which appears more than twenty times in the manuscript, generally in a relatively vague sense. The title restricts the approach to 'chaotic multiscale' problems and the Abstract extends this to 'chaotic, multi-scale, and transport-dominated problems'. One sentence in the Introduction identifies 'chaotic' with problems where 'every future state is unique', however deterministic problems containing transients also have this feature and nowhere is the effect of chaos explicitly demonstrated. Other descriptions of the applications of interest include those that exhibit 'slow decay of Kolmogorov N-width', those containing 'distributed multi-scale features,' and those with events 'intermittently distributed in both space and time'. The literature contains several approaches dealing with convection dominated problems containing a single isolated feature, most of which would appear to fail in problems with multiple and/or distributed features such as those addressed in this paper. I would strongly suggest replacing 'chaotic multi-scale' in the title with 'distributed multi-scale'. The comment about 'every future state is unique' should be retained as it is an important limitation for reduced order models, but I would recommend removing most other occurrences of the word and focus on problems with distributed multi-scale features as contrasted with those containing a single isolated feature.

\addrTwo{We agree with the reviewer. We feel that 'distributed multi-scale', 'transient' and 'unique future states' are more precise. We feel that just using one of them - say 'distributed' - many be weaker and less representative, and also leave the impression that this technique is meant for a specific problem. Clearly,  using all the words in the title would be an overkill given the already long title. As a compromise, we have retained chaotic in the title, but removed most instances in the main text and used your suggestions.}


The multiple forms of the variable q (no superscript or subscript, subscript r, superscript tilde, caret, and overbar) become difficult to follow and appear to be used inconsistently. A table midway through the manuscript that precisely defines the various nuances would help. Apparent inconsistencies in the notation occur in Section 4.1: Eq 18-20 use qr for the resolved modes, while Eq 21 and 22 use qr-bar for resolved modes and qr no longer appears. Then, in eq 25 q-caret is used for the full state ('the variable in eq 17') and is not defined until eq 39 where it appears to refer to the estimated full state variables from the adaptive basis.

\addrTwo{We thank the reviewer for pointing this out. We have switched to another symbol $\linearFOM$ in sec 4.1 to avoid the inconsistencies in notations and also highlighted each symbol in the revised version.}


The parameter, I - del-t*J first appears in eq 11 and then subsequently in eqs 18-22 after which it is often, but now always, replaced by B. The complexity of these latter expressions justify the simpler notation, but introducing B in eq 18 (or even in eq 11) would make the development easier to follow. Using B consistently would also nearly obviate the need for App B1, though it would remain useful.

\addrTwo{Following the reviewer's suggestion, we have revised Eqs.(18)-(25) with $\mathbf{B} \triangleq \mathbf{I} - \dt \mathbf{J}$ introduced earlier in Eq.(18).}



\textbf{Some more minor comments}:

Pg 3 Finite element methods with p>1 have multiple DOFs per element so the while the authors' definition of number of DOFs is appropriate for finite difference or finite volume it must be modified for finite element.

\addrTwo{Fixed on Pg 3.}


Distinguishing P and H (eq 5 and 8) is difficult. An explicit statement (line before Eq 6) that the norm is based on components of the mapped state variable $q_p$ should be added. Such a statement is present before Eq 9 indicating that the norm is based on the conservative variables, q. Also, since Eq 9 is identical to Eq 6. Remove eq 9 and reference eq 6.

\addrTwo{Fixed.}


Eq 12 constitutes a full reconstruction at all (not just non-sampled) elements

\addrTwo{Fixed.}


Below eq 15: I do not see how $S^T*U+$ can be computed offline since S and U vary during the computation.

\addrTwo{It can be computed offline for static-basis ROM but for adaptive ROM, it needs to be recomputed online. We have made a revision there to reflect this point.}


The algebraic expression two lines below eq 19 is missing a del-t

\addrTwo{Added.}


Adding a phrase between eq 23 and 24 would help

\addrTwo{Added.}

There is a sign error in eq 26

\addrTwo{Fixed.}


The vectors S and S* defined before eq 25 are complementary but vectors cannot be related by the identity matrix. The expression in App B4 properly relates the matrices $SS^T$ and $S*S*^T$.

\addrTwo{Fixed.}


In eq 3, the reduced state contains $n_p$ modes; in eq 18 it contains p modes.

\addrTwo{Fixed.}


==> StandardROM.tex <==
\section{Standard Model Reduction}
\label{StandardROM}
In this section, we introduce the standard Galerkin and least-squares Petrov-Galerkin (LSPG) projection methods for developing ROMs of the governing equations in Eq.~\ref{cfd:discretized}. 

\subsection{Construction of Proper Orthogonal Decomposition Bases} %for Conservative Variables}
\label{pod:consv}
In both approaches, the state $\solConsFOM$ is expressed in a trial space $\trialSpaceCons \triangleq \text{Range}(\trialBasisCons)$, where $\trialBasisCons \in \mathbb{R}^{\numDOF \times \numSolModes}$ is the trial basis matrix. We define $\solConsFOMRef(\timeVar) \triangleq \solConsFOM(\timeVar) - \solConsFOMRef$, where $\solConsFOMRef$ is a reference state. Possible reference states include the initial FOM solution, $\solConsFOMRef = \solConsFOM(\timeVar = \timeVar_0)$, or the time-averaged FOM solution, $\solConsFOMRef = \frac{1}{\Delta \text{T}} \int_{\timeVar_0}^{\timeVar_0 + \Delta \text{T}} \solConsFOM(\timeVar) \text{dt}$. 

We then seek a representation  $\solConsROMFull: [0,T] \rightarrow \trialSpaceCons$ such that
\begin{equation}
   \scaleMatCons \lp \solConsROMFull(\timeVar) - \solConsFOMRef \rp = \trialBasisCons \solConsROMRed(\timeVar),
    \label{pod:expansion_consv}
\end{equation}
where $\solConsROMRed: [0,T] \rightarrow \mathbb{R}^{\numSolModes}$ is the reduced state with $\numSolModes$ representing the number of trial basis modes. In this work, $\trialBasisCons$ is computed via the proper orthogonal decomposition (POD)~\cite{Lumley1997} from the singular value decomposition (SVD), which is a solution to
\begin{equation}
  \min_{\trialBasisCons \in \mathbb{R}^{\numDOF \times \numSolModes}} ||\dataMatCons - \trialBasisCons \trialBasisCons^T \dataMatCons ||_F\ \ s.t. \ \ \trialBasisCons^T \trialBasisCons = \mathbf{I},
    \label{pod:orthogonality_consv}
\end{equation}
Here, $\dataMatCons$ is a data matrix in which each column is a snapshot of the solution $\solConsFOMUnst$ at different time instances. A scaling matrix, $\scaleMatCons \in{\mathbb{R}^{\numDOF \times \numDOF}}$, must be applied to $\solConsFOMUnst$ such that the variables corresponding to different physical quantities in the data matrix $\dataMatCons$ have similar orders of magnitude. Otherwise, $\dataMatCons$ may be biased by physical quantities of higher magnitudes (e.g. total energy). In this work, we normalize all quantities by their $L^2$-norm, as proposed by Lumley and Poje~\cite{Lumley1997}
\begin{equation}
    \scaleMatCons = diag \lp \scaleMatCons_1, \ldots, \scaleMatCons_i, \ldots, \scaleMatCons_{\numElements} \rp,
    \label{pod:normalization_consv}
\end{equation} 
where $\scaleMatCons_i = diag\left( \varphi^{-1}_{1,norm}, \ldots , \varphi^{-1}_{\numVars,norm} \right)$. Here, $\varphi_{\normVarIdx,norm}$ represents the $\normVarIdx^{th}$ state  variable and
\begin{equation}
    \varphi_{\normVarIdx,norm} = {\frac{1}{\Delta \text{T}}\int^{t_0 + \Delta T}_{\timeVar_0} \frac{1}{\Omega} \int_{\Omega} \varphi'^2_\normVarIdx(\mathbf{x}, \timeVar) \; \text{d}\mathbf{x} \; \text{dt}}.
\end{equation} 


\subsection{Galerkin Projection}
\label{galerkin_rom}
Model reduction via Galerkin projection is formulated for the continuous-time representation of the FOM (Eq.~\ref{cfd:discretized}). This is done by first scaling Eq.~\ref{cfd:discretized} using the scaling matrix $\scaleMatCons$, then projecting onto the test space $\trialSpaceCons$
\begin{equation}
    \trialBasisCons^T \scaleMatCons \frac{\text{d} \solConsFOM}{\dTimeVar} = \trialBasisCons^T \scaleMatCons \rhsFunc{\solConsFOM, \timeVar}.
    \label{rom:galerkin}
\end{equation}
This specification that the trial and test spaces are identical defines Galerkin projection. The scaling of Eq.~\ref{cfd:discretized} is necessary to ensure that each equation makes similar contributions to the reduced system after projection. Otherwise, the reduced system may be biased by equations for quantities of higher magnitudes (e.g. the energy equation), exacerbating floating-point errors. With the low-rank representation in Eq.~\ref{pod:expansion_consv}, $\solConsROMFull(\timeVar) \triangleq \solConsFOMRef+\scaleMatCons^{-1}\trialBasisCons \solConsROMRed(\timeVar)$, substituted into Eq.~\ref{rom:galerkin}, a reduced-order ODE system can be obtained 
\begin{equation}
    \frac{\text{d}{\solConsROMRed}}{\dTimeVar} = \trialBasisCons^T \scaleMatCons \rhsFunc{\solConsROMFull, \timeVar}, \ \ \solConsROMRed(0) = \trialBasisCons^T\solConsFOM_0.
    \label{rom:galerkin_ode}
\end{equation}
 The dimension of the ROM ODE is $\numSolModes$, which can be orders of magnitudes smaller than  $\numDOF$  in Eq.~\ref{cfd:discretized}.

\subsection{Least-squares Petrov-Galerkin Projection}
\label{slspg_rom}
Least-squares Petrov-Galerkin (LSPG) projection~\cite{Carlberg2017} is formulated from the discrete-time representation of Eq.~\ref{cfd:discretized}. The objective of LSPG is to minimize the fully-discrete FOM equation residual, $\res$, defined in Eqs.~\ref{EqRes:LinearMultiStep} and~\ref{EqRes:RK}, with respect to the state, $\solConsFOM$, as approximated in the trial space $\trialSpaceCons$,  $\solConsROMFull = \solConsFOMRef + \scaleMatCons^{-1} \trialBasisCons \solConsROMRed$.
The problem statement of LSPG is to seek a solution to the minimization problem
\begin{equation}
    \solConsROMFull^\iterIdx \triangleq  \argmin_{ \solConsROMFull^\iterIdx \in \textrm{Range}(\trialBasisCons)} \norm{\scaleMatCons \resFunc{\solConsROMFull^\iterIdx}}^2,
    \label{rom:slspg_def}
\end{equation}
with the equation residual, $\res$, scaled by $\scaleMatCons$ such that each equation in $\res$ has similar contributions to the minimization. The norm used is the the Euclidean vector-induced matrix norm $L_{2,2}$, which we will represent by $\norm{\cdot}.$

The solution of this minimization problem seeks to satisfy
\begin{equation}
    \lp \testBasisCons^\iterIdx \rp^T \scaleMatCons \resFunc{\solConsROMFull^\iterIdx} = \zeroVec,
    \label{rom:slspg_proj}
\end{equation}
where $\testBasisCons^{\iterIdx}$ is the Petrov-Galerkin projection test basis given by
\begin{equation}
    \testBasisCons^\iterIdx = \frac{\partial \scaleMatCons \resFunc{\solConsROMFull^\iterIdx}}{\partial \solConsROMRed^\iterIdx}.
    \label{rom:slspg_w}
\end{equation}

For linear multi-step methods, the equation residual in Eq.~\ref{EqRes:LinearMultiStep} yields the test basis
\begin{equation}
    \testBasisCons^\iterIdx = \scaleMatCons \lp \mathbf{I} - \dt \beta_0 \jacobConsROM^\iterIdx \rp \scaleMatCons^{-1} \trialBasisCons,
    \label{rom:slspg_w_LinearMultistep}
\end{equation}
where $\jacobConsROM^\iterIdx = \left[\partial \rhs / \partial \solConsFOM \right]^\iterIdx_{\solConsFOM = \solConsROMFull}$. For explicit schemes ($\beta_0 = 0$), $\testBasisCons^\iterIdx = \trialBasisCons$, thus reverting to Galerkin projection. Similarly, for Runge--Kutta methods, the equation residual in Eq.~\ref{EqRes:RK} yields the test basis
\begin{equation}
    \testBasisCons^\iterIdx = \trialBasisCons,
    \label{rom:slspg_w_RK}
\end{equation}
for explicit and diagonally implicit schemes, which is identical to the trial basis as in Galerkin projection. For implicit Runge--Kutta methods,
\begin{equation}
    \testBasisCons^\iterIdx = \scaleMatCons \lp \mathbf{I} - \dt b_s \jacobConsROM^\iterIdx \rp \scaleMatCons^{-1} \trialBasisCons.
    \label{rom:slspg_w_RK_imp}
\end{equation}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
 
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}
